IM-Unpack: Training and Inference with Arbitrarily Low Precision Integers

GEneral Matrix Multiply (GEMM) is a central operation in deep learning and corresponds to the largest chunk of the compute footprint. Therefore, improving its efficiency is an active topic of ongoing research. A popular strategy is the use of low bit-width integers to approximate the original entries in a matrix. This allows efficiency gains, but often requires sophisticated techniques to control the rounding error incurred. In this work, we first verify/check that when the low bit-width restriction is removed, for a variety of Transformer-based models, whether integers are sufficient for all GEMMs need -- for {\em both} training and inference stages, and can achieve parity with floating point counterparts. No sophisticated techniques are needed. We find that while a large majority of entries in matrices (encountered in such models) can be easily represented by {\em low} bit-width integers, the existence of a few heavy hitter entries make it difficult to achieve efficiency gains via the exclusive use of low bit-width GEMMs alone. To address this issue, we develop a simple algorithm, Integer Matrix Unpacking (IM-Unpack), to {\em unpack} a matrix with large integer entries into a larger matrix whose entries all lie within the representable range of arbitrarily low bit-width integers. This allows {\em equivalence} with the original GEMM, i.e., the exact result can be obtained using purely low bit-width integer GEMMs. This comes at the cost of additional operations -- we show that for many popular models, this overhead is quite small.

==> figures/bf16-count.tex <==
\begin{figure}[!htbp]
\centering
% \vspace{-0.1in}
\includegraphics[width=0.4\textwidth]{files/bf16-count.pdf}
% \vspace{-0.3in}
\caption{Histogram of BF16 encoding. }
\label{fig:bf16_encode}
% \vspace{-0.05in}
\end{figure}


==> sections/evaluations.tex <==

\subsection{Training}

\subsection{Inference}


==> sections/matmul.tex <==

% Matrix multiplications are the essential operations in modern deep neural networks (we can view a convolution as a matrix multiplication as well). Given two matrices $\mA$ and $\mB$ of size $n \times d$ and $h \times d$ respectively, the output of a matrix multiplication is calculated via
% \begin{equation}
% \mC = \mA \mB^\T
% \end{equation}
% This operation usually represents the heaviest computation in both forward pass and backward pass of a deep neural network compared to are other operations such as non-linear activation and normalization. In the case of Transformers, for a linear layer, $\mA$ represents the inputs and $\mB$ is the parameter matrix. For self-attention computation, $\mA$ and $\mB$ represents the queries and keys respectively or the self-attention matrix and values. 

% Many work have been devoted to reduce the compute cost of this matrix multiplication. 
% For example, quantization
% pruning
% sparse computation
